Non-Euclidean Gradient Descent Operates at the Edge of Stability

The Edge of Stability (EoS) is a phenomenon where the sharpness (largest eigenvalue) of the Hessian approaches and then hovers near the stability threshold $2/\eta$ during gradient descent (GD) with step size $\eta$. Despite (apparently) violating classical smoothness assumptions, EoS has been widely observed in deep learning, but its theoretical foundations remain incomplete. We provide an interpretation of EoS through the lens of Directional Smoothness [Mishkin et al., 2024]. This interpretation naturally extends to non-Euclidean norms, which we use to define generalized sharpness under an arbitrary norm. Our generalized sharpness measure includes previously studied vanilla GD and preconditioned GD as special cases, as well as methods for which EoS has not been studied, such as $\ell_{\infty}$-descent, Block CD, Spectral GD, and their normalized versions. Through experiments on neural networks, we show that non-Euclidean GD with our generalized sharpness also exhibits progressive sharpening followed by oscillations around or above the threshold $2/\eta$. Practically, our framework provides a geometry-aware spectral diagnostic that can be applied across a broad class of non-Euclidean gradient methods.

==> macros.tex <==
\RequirePackage{xcolor}
\usepackage{amsmath,amsthm}
\usepackage{comment}
\usepackage{multirow}
%\usepackage{cite}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{threeparttable}
\usepackage{makecell}
\newcommand{\makecellnew}[1]{{\renewcommand{\arraystretch}{0.8}\begin{tabular}{c} #1 \end{tabular}}}

\usepackage[english]{babel}
\usepackage{amssymb}

\usepackage{bbm}
\usepackage{nicefrac}
\usepackage{lmodern}
%\usepackage[flushleft]{threeparttable}
\usepackage{epigraph}
\usepackage{subcaption}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{geometry}
\geometry{left=2.5cm}
\geometry{right=2cm}
\geometry{top=2cm}
\geometry{bottom=2cm}

\usepackage{etoc}


\RequirePackage{xcolor}
\usepackage{amsthm}
\usepackage{amsmath, amssymb}
\usepackage{comment}
\usepackage{multirow}
%\usepackage{cite}
%\usepackage[square,numbers]{natbib}
%\usepackage{graphicx}
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
%\usepackage{pifont}%for defining \xmark

\usepackage{etoc}


\usepackage[english]{babel}
%\usepackage{bbm}
\usepackage{nicefrac}
%\usepackage[flushleft]{threeparttable}
\usepackage{epigraph}
\usepackage{subcaption}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{breqn}


\usepackage[english]{babel}
%\usepackage{bbm}
\usepackage{nicefrac}
%\usepackage[flushleft]{threeparttable}
\usepackage{epigraph}
\usepackage{subcaption}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{breqn}

\usepackage{thm-restate}
\usepackage{empheq}
%\usepackage{bbold}
%\usepackage{dsfont}
\usepackage{authblk}
\usepackage{color}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\newcommand{\purple}{\color{purple}}
\newcommand{\teal}{\color{teal}}
\newcommand{\algnametitle}[1]{{\sf#1}}
\usepackage[pagebackref]{hyperref}
\hypersetup{
	colorlinks=true,        % false: boxed links; true: colored links
	linkcolor=blue,         % color of internal links
	filecolor=magenta,
	citecolor=darkgreen,         % color of links to bibliography
	urlcolor=blue           % color of external links
}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2)}%
    \else      \footnotesize{(Cited on pages~#2)}%
    \fi}

% \usepackage{cite}
\usepackage{framed}
\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage{algpseudocode}
\usepackage{enumerate}
\usepackage{thmtools}
\usepackage{wrapfig}

\def\toptitlebar{\hrule height1pt \vskip .25in} 
\def\bottomtitlebar{\vskip .22in \hrule height1pt \vskip .3in}

\graphicspath{{figs/}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bmm}{\mathbf{m}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\step}{\mbox{H}}
\newcommand{\bt}{\mathbf{\theta}}
\newcommand{\red}[1]{\textcolor[rgb]{0.635,0.0780,0.1840}{#1}}

%\newcommand{\algname}[1]{\texttt{#1}}
\newcommand{\algname}[1]{{\fontfamily{cmtt}\selectfont #1}}

\newcommand{\EoS}{{\algname{EoS}} }

\newcommand{\blue}[1]{\textcolor[rgb]{0,0.33,0.56}{#1}}
\newcommand{\green}[1]{\textcolor[rgb]{0,0.65,0.33}{#1}}
\definecolor{shade}{rgb}{0.9,0.9,0.9}
\usepackage{bm}
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
%\newcommand{\EOS}{\texttt{EoS}}
\newcommand{\EOS}{{\fontfamily{cmtt}\selectfont EOS}}
%% Robert commands
\newcommand{\norm}[1]{\left\| #1\right\|} 
\newcommand{\dotprod}[1]{\left< #1\right>} 
%\DeclareMathOperator*{\argmininn}{argmin} 
%\DeclareMathOperator*{\argmaxinn}{argmax} 
%\newcommand{\argmin}[1]{ \ensuremath{\underset{#1}{\argmininn} }\;}
%\newcommand{\argmax}[1]{ \ensuremath{\underset{#1}{\argmaxinn}}\;}
%\newcommand{\argmin}[1]{ \argmininn\;}
%\newcommand{\argmax}[1]{ \argmaxinn\;}
%\DeclareMathOperator*{\argmininn}{argmin}
%\DeclareMathOperator*{\argmaxinn}{argmax}
%\newcommand{\argmin}[1]{\ensuremath{\underset{#1}{\argmininn}\;}}
%\newcommand{\argmax}[1]{\ensuremath{\underset{#1}{\argmaxinn}\;}}
\usepackage{amsmath}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}





\newcommand{\cN}{\mathcal{ N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cS}{\mathcal{ S}}
\newcommand{\mD}{\mat{ D}}
\newcommand{\mG}{\mat{ G}}
\newcommand{\mH}{\mat{ H}}
\newcommand{\mP}{\mat{ P}}
\newcommand{\mM}{\mat{ M}}
\newcommand{\mA}{\mat{ A}}
\newcommand{\mU}{\mat{ U}}
\newcommand{\mV}{\mat{ V}}
\newcommand{\mX}{\mat{ X}}
\newcommand{\mW}{\mat{ W}}
\newcommand{\DW}{\mat{ \Delta W}}
\newcommand{\mI}{\mat{ I}}
\newcommand{\mS}{\mat{ \Sigma}}
\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator{\traceOp}{tr}  
\newcommand{\trace}[1]{\traceOp\left(#1\right)}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right] } 
\newcommand{\EE}[2]{\mathbb{E}_{#1}\left[#2\right] }

\newcommand{\cW}{\mathcal{ W}}
\usepackage{amsthm}
\usepackage{amsbsy}

\usepackage{mathtools}

\usepackage{mdframed} 
\usepackage{thmtools}
\newif\ifappendix

\definecolor{shadecolor}{gray}{0.90}
\declaretheoremstyle[
headfont=\normalfont\bfseries,
notefont=\mdseries, notebraces={(}{)},
bodyfont=\normalfont,
postheadspace=0.5em,
spaceabove=6pt,
mdframed={
  skipabove=8pt,
  skipbelow=8pt,
  hidealllines=true,
  backgroundcolor={shadecolor},
  innerleftmargin=4pt,
  innerrightmargin=4pt}
]{shaded}


\declaretheorem[style=shaded,within=section]{definition}
\declaretheorem[style=shaded,sibling=definition]{theorem}
\declaretheorem[style=shaded,sibling=definition]{proposition}
\declaretheorem[style=shaded,sibling=definition]{assumption}
\declaretheorem[style=shaded,sibling=definition]{corollary}
\declaretheorem[style=shaded,sibling=definition]{conjecture}
\declaretheorem[style=shaded,sibling=definition]{lemma}
\declaretheorem[style=shaded,sibling=definition]{remark}
\declaretheorem[style=shaded,sibling=definition]{example}


\usepackage[most]{tcolorbox}  % in your preamble
\definecolor{myframecolor}{RGB}{0,60,125}
\colorlet{myframecolorlight}{myframecolor!20!white}
\tcbset{
  myremark/.style={
    colback=blue!5!white,
    colframe=myframecolorlight,
    coltitle=black,
    fonttitle=\bfseries,
    boxrule=0.8pt,
    arc=4pt,
    title=#1
  }
}

\allowdisplaybreaks
% Commenting
\usepackage[colorinlistoftodos]{todonotes}

% Custom inline todo commands with unique colors
\newcommand{\rob}[1]{\todo[inline,bordercolor=blue,backgroundcolor=blue!20,linecolor=blue]{\textbf{Robert: }#1}}
\newcommand{\rustem}[1]{\todo[inline,bordercolor=green!50!black,backgroundcolor=green!20,linecolor=green!50!black]{\textbf{Rustem: }#1}}
\newcommand{\jeremy}[1]{\todo[inline,bordercolor=red,backgroundcolor=red!20,linecolor=red]{\textbf{Jeremy: }#1}}
\newcommand{\michael}[1]{\todo[inline,bordercolor=purple,backgroundcolor=purple!20,linecolor=purple]{\textbf{Michael: }#1}}



%\usepackage[hidelinks]{hyperref}

%\usepackage[firstinits=true,backend=bibtex,style=alphabetic,citestyle=alphabetic, url =false, arxiv =false, isbn = false, doi = false]{biblatex}
%\bibliography{references}
\usepackage[pagebackref]{hyperref}
\usepackage[nameinlink]{cleveref}
\hypersetup{
	colorlinks=true,        % false: boxed links; true: colored links
	linkcolor=blue,         % color of internal links
	filecolor=magenta,
	citecolor=darkgreen,         % color of links to bibliography
	urlcolor=blue           % color of external links
}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2)}%
    \else      \footnotesize{(Cited on pages~#2)}%
    \fi}


\hypersetup{colorlinks, citecolor=blue, filecolor=black, urlcolor=blue}
%%%%%%%%%%%

%\usepackage{titlesec}
\definecolor{sectionblue}{RGB}{0,60,125}
%\titleformat{\section}{\normalfont\Large\bfseries\color{sectionblue}}{\thesection}{1em}{}
%\titleformat{\subsection}{\normalfont\large\bfseries\color{sectionblue}}{\thesubsection}{1em}{}
